Variational Offline Multi-agent Skill Discovery

Skills are effective temporal abstractions established for sequential decision making, which enable efficient hierarchical learning for long-horizon tasks and facilitate multi-task learning through their transferability. Despite extensive research, research gaps remain in multi-agent scenarios, particularly for automatically extracting subgroup coordination patterns in a multi-agent task. In this case, we propose two novel auto-encoder schemes: VO-MASD-3D and VO-MASD-Hier, to simultaneously capture subgroup- and temporal-level abstractions and form multi-agent skills, which firstly solves the aforementioned challenge. An essential algorithm component of these schemes is a dynamic grouping function that can automatically detect latent subgroups based on agent interactions in a task. Further, our method can be applied to offline multi-task data, and the discovered subgroup skills can be transferred across relevant tasks without retraining. Empirical evaluations on StarCraft tasks indicate that our approach significantly outperforms existing hierarchical multi-agent reinforcement learning (MARL) methods. Moreover, skills discovered using our method can effectively reduce the learning difficulty in MARL scenarios with delayed and sparse reward signals. The codebase is available at https://github.com/LucasCJYSDL/VOMASD.

==> related_works.tex <==
\section{Related Works} \label{rw}

In this section, we provide a comprehensive review on the use of skills in cooperative MARL, and emphasize the novelty of our proposed algorithm. We categorize these works into several groups based on their algorithm designs. The first group of works either rely on predefined skills \cite{DBLP:conf/atal/AmatoKK14,DBLP:journals/jair/AmatoKKH19} or require well-designed task hierarchies/decomposition \cite{DBLP:conf/imsccs/ShenGL06,DBLP:journals/aamas/GhavamzadehMM06,fosong2023learning}. However, we focus on automatic task decomposition and skill discovery, which is more demanding but makes our algorithm more applicable. Next, we introduce research works in this direction.

% In particular, we categorize these works into four groups based on their algorithm designs as follows. The differences between algorithms across these categories are subtle yet understanding these distinctions is crucial, as they inspire the direction of algorithm development.

A straightforward manner is to learn a set of single-agent skills for each agent using discovery methods proposed in single-agent scenarios \cite{DBLP:conf/iclr/EysenbachGIL19,DBLP:conf/iclr/JinnaiPMK20,DBLP:conf/nips/ChenAL23,DBLP:journals/corr/abs-2305-17327}, and then learn a multi-agent meta policy over these individual skills. The intuition is that players in a team sport can master their skills individually outside of team practices.
% and afterwards it would be easier for these skilled players to manage complex team tasks. 
Specifically, the meta policy $\pi_h(\vec{z}\mid s)$ assigns skills $\vec{z}=(z^1, \cdots, z^n)$ to all agents, and then each agent decides on its primitive action according to its skill policy $\pi_l(a^i\mid \tau^i, z^i)$. Note that (1) $z^i \in \Omega^z$ is an embedding of a single-agent skill and $\Omega^z$ is a finite set of skill choices; (2) $\pi_h(\vec{z}\mid s)$ is usually implemented as $(\pi_h^1(z^1\mid \tau^1), \cdots, \pi_h^n(z^n\mid \tau^n))$ in CTDE schemes to enable decentralized skill selection. 
% \footnote{The meta policy $\pi_h^{1:n}$ is trained in a centralized manner, so the global state information is taken into consideration by the team for the skill selection, even though each agent $i$ only uses its own view as the input.}. 
Representative works of this category include \cite{DBLP:conf/iclr/LeeYL20,DBLP:conf/atal/YangBZ20,DBLP:conf/gecco/SachdevaKMT21}. In \cite{DBLP:conf/iclr/LeeYL20}, skills $\pi_l$ are learned in a separate stage, while, in \cite{DBLP:conf/atal/YangBZ20,DBLP:conf/gecco/SachdevaKMT21}, skills are concurrently trained with the meta policy $\pi_h$. Typically, as in single-agent scenarios, the skill duration $H$ is a predefined value, and a new skill assignment for all agents, i.e., $\vec{z}$, should be given by the meta policy every $H$ time steps. However, some algorithms \cite{DBLP:conf/atal/ChakravortyWRCB20,DBLP:conf/nips/XiaoTA22,DBLP:conf/kdd/Zhang0LW023} have been proposed for the case where the skills of each agent can take different amounts of time and so the skill selection across agents can be asynchronized. 
% These algorithms are more complicated in design; especially, \cite{DBLP:conf/atal/ChakravortyWRCB20} is based on the option framework \cite{DBLP:journals/ai/SuttonPS99} where each agent needs to additionally learn a termination policy to decide on when to terminate a skill. 
To sum up, this group of works replace the primitive action set $A$ in MARL with an individual-skill set $\Omega^z$, which could simplify the learning especially for long-horizon tasks. 
% Further, each skill can be used in various subtasks without relearning to improve the training efficiency. 
However, in multi-agent scenarios, discovering inter-agent coordination patterns as multi-agent skills is possible. Learning with multi-agent skills could be simpler, since they constitute higher-level abstractions of multi-agent behaviors than single-agent skills and are closer in form with the overall multi-agent policy.
% which constitutes higher-level abstractions of the multi-agent interaction experience and can further simplify the learning of the overall multi-agent policy.

Another main branch of algorithms is role-based MARL. These algorithms, based on the CTDE scheme, usually contain three modules: establishing role representations $\Omega^Z = \{Z_1, \cdots, Z_m\}$, learning a role selector $\pi_h(Z^i\mid \tau^i)$ 
% \footnote{The role selectors of each agent $\pi_h^i(Z^i\mid \tau^i)$ ($i=1, \cdots, n$) usually would share their parameters, so we denote the role selector as $\pi_h(Z^i\mid \tau^i)$.} 
($Z^i \in \Omega^Z$), and learning role policies $\pi_l(a^i\mid \tau^i, Z^i)$.
% where $m$ is the predefined number of roles. 
This framework is similar with the one used for MARL with single-agent skills. However, the policy of role $Z$, i.e., $\pi_l(a^i\mid \tau^i, Z)$, is not a single-agent skill policy but a policy for the subgroup $g_Z$. This is because each agent $i \in g_Z$ adopts the same role policy $\pi_l(\cdot\mid \cdot, Z)$ and $\pi_l(\cdot\mid \cdot, Z)$ is trained in a centralized manner with the aim for the subgroup $g_Z$ to maximize a global return. As a comparison, aforementioned \cite{DBLP:conf/iclr/LeeYL20,DBLP:conf/gecco/SachdevaKMT21} learn skill policies $\pi_l(\cdot\mid \cdot, z)$ based on reward functions specifically defined for single-agent skills, and \cite{DBLP:conf/atal/YangBZ20} updates skill policies through Independent Q-learning, i.e., a fully-decentralized training scheme, thus the learned skills are for individuals. Notable works in this category, roughly ordered by the publication date, include \cite{DBLP:conf/icml/0001DLZ20,DBLP:conf/icml/LiuLSGZA21,DBLP:conf/iclr/00010MPWZ21,DBLP:conf/nips/LiuLXDL22,DBLP:conf/nips/IqbalCS22,DBLP:conf/nips/Yang0HZZL22,li2023celebrating,DBLP:conf/nips/ZangHLFFXC23,DBLP:conf/nips/TianCHLZWPGDGC23,DBLP:conf/aaai/XuBZ0F23,xia2023dynamic,zhou2024constructing}. Among these works, $Z$ is given different names, such as role \cite{DBLP:conf/icml/0001DLZ20}, ability \cite{DBLP:conf/nips/Yang0HZZL22}, subtask \cite{li2023celebrating}, and skill \cite{DBLP:conf/nips/LiuLXDL22}, but refers to the same concept. All these works utilize a similar algorithm framework, which, as mentioned above, contains three modules for learning the role embedding, role selector\footnote{Most algorithms in this category adopt decentralized selectors, i.e., $(\pi_h(Z^1\mid \tau^1), \cdots, \pi_h(Z^n\mid \tau^n))$, but there are some works, such as \cite{DBLP:conf/icml/LiuLSGZA21,DBLP:conf/nips/IqbalCS22}, utilizing centralized ones, i.e., $\pi_h(\vec{Z}\mid s)$. 
% but makes it less flexible than fully-decentralized execution
The global state could provide more information for the coordinated role assignment.}, and role policy, respectively. One main distinction lies in their varied approaches for learning the role embedding, which can be based on action effects \cite{DBLP:conf/iclr/00010MPWZ21}, global state reconstruction \cite{zhou2024constructing}, or predictions of the next observation and reward \cite{DBLP:conf/nips/LiuLXDL22}. 
% or automatic grouping results \cite{DBLP:conf/nips/ZangHLFFXC23}. 
% Besides maximizing the global return, regularization terms are often employed for optimizing those three components. For example, diversity is encouraged in the learned role embeddings, and temporal consistency is regulated in the role selection process to avoid frequent changes in role assignments over time.
% and role specialization is promoted through regularizing the role policy with a mutual information term between the role and its corresponding policy trajectory $I(\tau;Z)$. 
% These regularizers are shown to be essential for learning performance and different works in this category vary in the regularizer design. 
As a recommendation, readers who are new to this area can refer to the two representative works: \cite{DBLP:conf/nips/Yang0HZZL22,DBLP:conf/aaai/XuBZ0F23}. 
% Most algorithms in this category are extended on value decomposition MARL methods like QMIX, thus $\pi_h(Z^i\mid \tau^i)$ and $\pi_l(a^i\mid \tau^i, Z^i)$ are implemented as Q-networks. \cite{DBLP:conf/nips/Yang0HZZL22,DBLP:conf/aaai/XuBZ0F23} represent two manners for this extension, either viewing $(\pi_h, \pi_l)$ as a unified policy and adopting a single mixing network for it or using two mixing networks for $\pi_h, \pi_l$ respectively. 
To sum up, although the role policy $\pi_l(a^i\mid \tau^i, Z)$ is more than a single-agent skill and learned as a subgroup policy for $g_Z$, agents in $g_Z$ are similar in behaviors as they all adopt a policy conditioned on $Z$. As mentioned in 
% share the same role in a task and
% \cite{DBLP:conf/icml/0001DLZ20}, for any two agents, either they have similar roles or they have quite different behaviors; also, in 
\cite{DBLP:conf/nips/Yang0HZZL22}, role-based MARL is designed to group agents with similar abilities into the same subtask. However, multi-agent skills should be abstractions of subgroup coordination patterns, and agents from this subgroup could possess heterogeneous behaviors. For instance, the collaboration between two pilots -- one proficient in advanced flying maneuvers and the other in weapon control -- while operating a fighter jet, exemplifies a multi-agent skill. Therefore, the concept of a multi-agent skill is more generalized than that of role policy and cannot be acquired through aforementioned role-based algorithms.

There are relatively few works on multi-agent skill discovery. The authors of \cite{DBLP:journals/corr/abs-2006-04021,DBLP:conf/nips/ChenCLA22,DBLP:conf/nips/Yang0LZL23} propose algorithms to discover skills for the entire team of agents. As a representative, in \cite{DBLP:conf/nips/Yang0LZL23}, they adopt a transformer-based skill selector $\pi_h(z^{1:n}, Z\mid s)$ to decide on the team skill $Z$ and individual skills $z^{1:n}$ autoregressively
% in the order of $Z, z^1, \cdots, z^n$ 
based on the global state. Then, each agent $i$ interacts with the environment using a corresponding policy $\pi_l(a^i\mid \tau^i, z^i, Z)$\footnote{In \cite{DBLP:conf/nips/Yang0LZL23}, $Z$ is not used as a condition of $\pi_l$ but adopted for centralized training, so the team skill information is implied in $\pi_l$.}. Compared with the role policy $\pi_l(\cdot\mid \cdot, Z)$, the team skill $\pi_l(\cdot\mid \cdot, z, Z)$ could contain heterogeneous behaviors across agents, which are embedded as various individual skills $z^{1:n}$. However, the team skill is only a special instance of multi-agent skills, as the number of agents within a team skill is always $n$. 
% Effective multi-agent skills should capture coordination patterns among agents, which usually occur within subgroups rather than the entire team, and team skills are less flexible to be utilized or transferred especially for big teams as it requires to coordinate all agent members. 
Ideally, multi-agent skill discovery should identify subgroups where agents interact frequently and extract their behavior patterns as joint skills, and the size of the subgroup could vary from 1 to $n$, which is much more challenging as it additionally requires dynamic grouping according to the task scenario. 
% Regarding the application of learned multi-agent skills, \cite{DBLP:journals/corr/abs-2006-04021} does not provide necessary details; while, in \cite{DBLP:conf/nips/Yang0LZL23}, the decision on \(z^i\) requires \(s\), \(Z\), and \(z^{1:i-1}\), which hinders decentralized execution. 
% Notably, there is another line of works \cite{chen2023multiagent,9847387,DBLP:conf/nips/ChenCLA22} that extend the Laplacian-based skill discovery \cite{DBLP:conf/iclr/JinnaiPMK20} from single-agent to multi-agent scenarios. However, these algorithms rely on estimations for the Laplacian spectrum of the joint-state transition graph of the agents, which restricts their applicability and scalability. In particular, these algorithms are mainly proposed and useful for goal-achieving tasks, and the computation cost to discover multi-agent options grows exponentially with the number of agents, so, at most, three-agent options are discovered and utilized in their experiments.

All the algorithms mentioned above are for \textbf{online} skill discovery, while the authors of \cite{DBLP:conf/iclr/ZhangJLY0Z23} propose an approach for discovering coordination skills from offline data. However, this algorithm is still a role-based one, 
% with a centralized role selector during training
 and the learned role policy $\pi_l(\cdot\mid \cdot, Z)$ is different from multi-agent skills in concept as mentioned above. The difference between \cite{DBLP:conf/iclr/ZhangJLY0Z23} and aforementioned role-based methods is that it replaces task rewards with the reconstruction accuracy of joint actions, so that the learned skills are not task-specific but generalizable. 
% Nevertheless, it's hard to ensure that the skills learned through single-step action reconstruction can extend temporally.
% Our work falls in the same task setting -- learning generalizable, multi-agent temporal abstractions from offline data, but focuses on a more challenging learning target -- multi-agent skills.

In conclusion, research on multi-agent skill discovery is still at an early stage of development, especially for the offline setting. Even without prelearned skills, when dealing with a complex multi-agent task, the agents would implicitly learn to decompose the overall task into several subtasks, assign a subgroup for each subtask, and develop a joint policy (i.e., multi-agent skill) within the subgroup to handle the corresponding subtask. Replacing primitive actions with single-agent skills or role policies could make such a learning process more efficient, as agents can assemble these higher-level abstractions to obtain the required subgroup joint policies more easily. As the first offline multi-agent skill discovery algorithm, our work takes one step further by directly identifying subgroups, which could change throughout a decision horizon, and extracting their coordination patterns as multi-agent skills. With these joint skills, the MARL process could be greatly simplified, since agents only need to select correct multi-agent skills without considering grouping with others or forming subgroup policies. Compared to single-agent skills or role policies, multi-agent skills make better use of the offline multi-agent interaction data, representing a more efficient form of knowledge discovery. 
% Moreover, the discovered skills can potentially be transferred across a distribution of tasks to simplify multi-task learning, since, as policy segments, these joint skills have better transferability than the overall multi-agent policy.

% A role policy can be viewed as a multi-agent skill where each agent utilizes the same single-agent skill. Multi-agent skills devides the decision horizon and cluster the pool of agents.
% Works that take generalization into consideration include \cite{DBLP:conf/icml/LiuLSGZA21,DBLP:conf/nips/TianCHLZWPGDGC23,DBLP:conf/iclr/ZhangJLY0Z23}.
